A Distributed Neural Network Architecture for Robust Non-Linear Spatio-Temporal Prediction

We introduce a distributed spatio-temporal artificial neural network architecture (DISTANA). It encodes mesh nodes using recurrent, neural prediction kernels (PKs), while neural transition kernels (TKs) transfer information between neighboring PKs, together modeling and predicting spatio-temporal time series dynamics. As a consequence, DISTANA assumes that generally applicable causes, which may be locally modified, generate the observed data. DISTANA learns in a parallel, spatially distributed manner, scales to large problem spaces, is capable of approximating complex dynamics, and is particularly robust to overfitting when compared to other competitive ANN models. Moreover, it is applicable to heterogeneously structured meshes.

==> outlook.tex <==
% Make the main file the master document for this file so that when compiling this file, actually the master file will be compiled. The name of the main file could also contain paths, like path/main.tex
% !TeX root = 2020-SpatioTemporalRNN.tex


\section{Outlook}

% Wenn die zusaetzlichen Autoren noch genug Platz lassen, denke ich, hier sollten noch 1-2-3 kurze Saetzen zu den wesentlichen Apspekten der Architektur stehen. Die Perspektive ist cool. ggf. sollten wir hier schon noch erwaehnen, dass wir das als naechstes auf Wetterdaten anwenden.

So far, we have only considered regularly distributed grid data, where distances between single measurement points are identical. However, this data situation is not given in many applications, such as neural information processing in the brain, traffic predictions on roads, or data propagation on graphs, where distances and the number of neighboring vertices vary to large extents.
Ongoing work shows that DISTANA can deal with irregularly distributed sensor meshes, making it applicable to arbitrarily, metrically-distributed graphs.

% Another promising research direction is to apply our model to the moving MNIST data set and compare performances.
